Partitioned Gradient Matching-based Data Subset Selection for Compute-Efficient Robust ASR Training

Training state-of-the-art ASR systems such as RNN-T often has a high associated financial and environmental cost. Training with a subset of training data could mitigate this problem if the subset selected could achieve on-par performance with training with the entire dataset. Although there are many data subset selection(DSS) algorithms, direct application to the RNN-T is difficult, especially the DSS algorithms that are adaptive and use learning dynamics such as gradients, as RNN-T tend to have gradients with a significantly larger memory footprint. In this paper, we propose Partitioned Gradient Matching (PGM) a novel distributable DSS algorithm, suitable for massive datasets like those used to train RNN-T. Through extensive experiments on Librispeech 100H and Librispeech 960H, we show that PGM achieves between 3x to 6x speedup with only a very small accuracy degradation (under 1% absolute WER difference). In addition, we demonstrate similar results for PGM even in settings where the training data is corrupted with noise.

==> GradMatch for Speech/results.tex <==

 \textbf{Datasets} We perform all our experiments on the Librispeech dataset~\cite{panayotov2015librispeech}. We present results on the medium-scale Librispeech 100H as well as on the large-scale Librispeech 960H datasets.


 Along with the standard Librispeech benchmark, we also perform experiments on noisy Librispeech, where the speech is augmented with noise across varying signal-to-noise ratios (up to 15db) on a fraction of the training data. We refer to this dataset as \textbf{Librispeech-noise}, where up to 30\% examples in the original dataset are augmented with noise across varying signal-to-noise ratios.
 
 \textbf{Architecture.} We perform all our experiments on the Speechbrain's\cite{ravanelli2021speechbrain} Librispeech transducer recipe. The transcription network of the RNN-T consists of a CRDNN encoder which has 2 CNN blocks followed by 4 layers of bi-LSTMs and subsequently followed by 2 DNN layers. The prediction network consists of an embedding layer followed by a single layer GRU unit. A joint network is a single linear layer that projects 1024 dimensional representations to output a vocabulary of 1000 BPE. The decoding is done through a time-synchronous decoding algorithm~\cite{graves2012sequence, hannun2019sequence} with a beam size of 4. The decoding involves an external transformer language model trained on the Librispeech corpus~\cite{kannan2018analysis,hrinchuk2020correction, wolf2019huggingface}.



% \begin{figure}
% \begin{center}
% \includegraphics[width = \columnwidth]{Figures/chart_1.png}
% \caption{WER results on Librispeech 100H.}
% \label{fig_1:wer}
% \end{center}
% \end{figure}


% \begin{figure}
% \begin{center}
% \includegraphics[width = \columnwidth]{Figures/chart_2.png}
% \caption{Relative Test Error vs Speed Up for subset selection methods on Librispeech 100H.}
% \label{fig_2}
% \end{center}
% \end{figure}

\begin{figure*}[!tb]
\centering
\begin{minipage}{.8\textwidth}
\resizebox{\columnwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{cl|ll|c}
\hline
\multicolumn{1}{l}{Subset} & Method                & \multicolumn{2}{c}{WER (Rel. Test Error) ($\downarrow$)} & Speed Up ($\uparrow$)             \\ \hline
\multicolumn{1}{l}{}            &                       & \textsc{test-clean}          & \textsc{test-other}          &                       \\ \hline \hline
\multicolumn{1}{l}{100\%}   & \multicolumn{1}{c|}{-} & 4.21 (0.0)          & 11.59 (0.0)         & \multicolumn{1}{c}{-} \\ \hline 
\multirow{2}{*}{10\%}           & \random          & 5.87 (39.43\%)      & 15.39 (32.79\%)     & 6.25                  \\
                                & \dsys            & 5.71 (35.63\%)      & 14.66 (26.49\%)     & 4.43                  \\ \hline \hline
\multirow{2}{*}{20\%}           & \random          & 5.08 (20.67\%)      & 13.89 (19.84\%)     & 3.95                  \\
                                & \dsys            & 5.01 (19\%)         & 12.78 (10.27\%)     & 3.30                  \\ \hline \hline
\multirow{2}{*}{30\%}           & \random         & 4.62 (12.65\%)      & 12.65 (9.74\%)      & 2.89                  \\
                                & \dsys            & 4.58 (8.79\%)       & 12.45 (7.42)        & 2.64                  \\ \hline
\end{tabular}}
\captionof{table}{\label{tab:wer_960}Results showing WER (Relative Test Error) and Speed Up on \textsc{test-clean} and \textsc{test-other} test splits of Librispeech 960H.}
%\vspace{.5cm}
\end{minipage}%
\hfill
\begin{minipage}{.9\textwidth}
  \centering
  \resizebox{\columnwidth}{!}{
\begin{tabular}{ll||cc||cc||cc}
\hline
                      & Subset & \multicolumn{2}{c}{Noise = 10\%} & \multicolumn{2}{c}{Noise = 20\%} & \multicolumn{2}{c}{Noise = 30\%} \\ \hline
                      &        & \random    & \dsys    & \random     & \dsys    & \random     & \dsys    \\ \hline \hline
\multirow{4}{*}{100H} & 100\%  & \multicolumn{2}{c||}{10.59}        & \multicolumn{2}{c||}{11.16}        & \multicolumn{2}{c}{11.39}        \\ 
                      & 10\%   & 11.79            & 11.86         & 11.64            & 11.67         & 11.96            & 11.82         \\
                      & 20\%   & 11.53            & 10.8          & 11.27            & \textbf{11.12}         & 11.39            & 11.25         \\
                      & 30\%   & 11.33            & \textbf{10.7}          & 11.74            & 11.42         & 12.05            & \textbf{11.17}         \\ \hline
\multirow{4}{*}{960H} & 100\%  & \multicolumn{2}{c||}{4.52}         & \multicolumn{2}{c||}{4.65}         & \multicolumn{2}{c}{4.68}             \\ 
                      & 10\%   & 6.5              & 6.28          & 6.44             & 6.54          & 6.58             & 6.43          \\
                      & 20\%   & 5.61             & 5.58          & 5.44             & 5.65          & 5.84             & 5.5           \\
                      & 30\%   & 4.99             & \textbf{4.97}          & 5.16             & \textbf{5.02}          & 5.62             &  \textbf{5.17} \\ \hline   
\end{tabular}}
\captionof{table}{\label{tab:wer_noise}Results showing WER on \textsc{test-clean} test set of  Librispeech 100H trained using noisy Librispeech dataset using \dsys{} and \random.}
%\vspace{-.65cm}
\end{minipage}
\end{figure*}


 \textbf{Training Details.} For the training, we employ a learning rate of 2.0 with an annealing factor of 0.8 for the relative improvement of 0.0025 on validation loss (sometimes referred to as newbob scheduler). The training on Librispeech 100H is performed on two A100 40GB GPUs with the effective batch size of 8, whereas for Librispeech 960H, we employ two A100 80GB GPUs with an effective batch size of 24. All the training is done for 30 epochs. In all our experiments, the \dsys{} algorithm is invoked after every $5^{th}$ epoch ($R = 5$) after performing warm-start (training on full data) for 7 and 2 epochs on Librispeech 100H and Librispeech 960H datasets respectively. The results for each setting are averaged over 3 runs with different random seeds.

\textbf{\dsys{} Details.} For doing the subset selection with \dsys{}, we use the gradients of the Joint Network parameters, which we believe would have the maximum information concentrated for the sequence. We freeze the rest of the network while we compute the gradient of the Joint Network of the RNN-T. We use $D=7$ and $D=50$ (data partitions) to obtain subsets using the \dsys{} algorithm over gradients of training data for Librispeech 100H and 960H datasets respectively. Subset selection is performed using \textbf{{\em training set loss gradients}} in experiments performed using Librispeech 100H (Figures~\ref{fig_1:wer},\ref{fig_2}) and Librispeech 960H (table \ref{tab:wer_960}). For experiments with \textbf{Librispeech-noise} (Table~\ref{tab:wer_noise}) we employ the \textbf{{\em validation gradients}} for performing the subset selection, {\em since we are also concerned with robustness in the presence of noise}. 

\textbf{Baselines.} We compare the results obtained using the \dsys{} method against three intuitive baselines - (i) \textbf{\random{}} baseline, in which the subset of the dataset is obtained by choosing points with uniform probability. (ii) \textbf{\largeOnly{}} - For each subset, we employ only the largest utterances based on duration. (iii) \textbf{\largeSmall{}} - For each subset size, half of the subset is filled with smallest utterances and the other half with the largest utterances based on duration, to remove the length bias of the \textbf{\largeOnly{}} baseline. %at every $5^{th}$ epoch to match the subset budget. \textbf{Random Online} is a stronger baseline then the usually reported \textbf{Random} baseline \cite{pmlr-v139-killamsetty21a} in which the subset is selected only once. \textbf{Random} experiences accuracy degradation of at least $1\%$ absolute WER difference over \textbf{Random Online}.

\subsection{Results}

To compare the efficacy of the \dsys, we compare the word error rate (WER), relative test error, and speed-up compared to  training with the entire dataset. We compute these metrics for both the Librispeech 100H and Librispeech 960H benchmarks.
Additionally, we also, present energy ratios {\em vs.} relative test error rate tradeoff on Librispeech 100H.
%Additionally, we also, present energy ratios for the entire Librispeech 900H dataset and relative test error rate tradeoff on Librispeech 100H. \todo{But why only "energy ratios for the entire dataset Librispeech 900H dataset and relative test error rate tradeoff on Librispeech 100H"?}

In Figure \ref{fig_1:wer}, we present the comparison of WER for \dsys{} against various baselines for various subset sizes of the full dataset. With just 20\% of the subset size, the \dsys{} method yields a WER of 10.66 as opposed to 10.08 obtained by training on the full dataset. For Librispeech 100H, \dsys{} consistently outperforms all the baseline, thus illustrating the effect 
%superiority 
of selecting subsets using the gradient matching algorithm. Also note, \random{} baseline is consistently better than other heuristic based baselines such LargeOnly and LargeSmall. In Figure~\ref{fig_2}, we plot the speed up against the Relative Test Error for Librispeech 100H. While \random{}  baseline is observed to attain higher speed up in comparison to the \dsys{} because of the simple selection strategy, \random{} baseline also incurs higher relative test error in comparison to the \dsys. 

In Figure \ref{fig4:energy}, we present the plot of relative test error {\em w.r.t} energy efficiency for the full training setting. We use pyJoules\footnote{https://pypi.org/project/pyJoules/} for measuring the energy consumed by GPU cores.  We show that with \dsys, the training time is halved and energy efficiency is doubled while incurring the relative test error of less than 5\% as compared to the training on the entire dataset. For higher speedups, where there is a degradation in the WER, the loss is relatively better for \dsys{} as compared to the baseline. We do not show the energy efficiency for LargeOnly and LargeSmall baselines as their relative test error is consistently poor as compared to the Random Subset baseline as shown in Figure~\ref{fig_2}.

\begin{figure}[!t]
\includegraphics[width = \columnwidth,height=5.5cm]{Figures/chart_3.png}
\caption{Energy Ratio($\uparrow$) {\em vs.} Relative Test Error($\downarrow$) for \dsys{} and \random{} on Librispeech 100H.}
\label{fig4:energy}
\end{figure}
%\todo[]{Durga: Please resize the Figure 4 to 1 column.}


\begin{figure*}[!tb]
\centering
\begin{minipage}{\columnwidth}
%\small{
\begin{tabular}{l|c|c}
\hline
                    & \random  & \multicolumn{1}{l}{\dsys} \\ 
                    \hline \hline
                
Overlap Index       & 20.2\%       & 6.37\%                         \\
Noise Overlap Index & 0.82\%        & 0.83\%               \\ \hline    \hline     
\end{tabular}%}
\captionof{table}{\label{tab:ablation-1} Overlap Indices - measures the overlap between consecutive subsets for \dsys{} and \random{} methods.}
%\vspace{-.65cm}
\end{minipage}%
\hfill
\begin{minipage}{\columnwidth}
  \centering
  \begin{tabular}{c|c|c}
\hline 
Subset Size & WS = 2 epochs & WS= 3 epochs \\ \hline \hline
10\%        & 5.71                  & 5.3                   \\
20\%        & 5.01                  & 4.82                  \\
30\%        & 4.58                  & 4.54                 \\ \hline \hline
\end{tabular}
\captionof{table}{\label{tab:ablation-2} Effect of warm-start (WS) on WER for PGM on \textsc{test-clean} test set for Librispeech 960H}
%\vspace{-.65cm}
\end{minipage}
\end{figure*}

\begin{table}[!t]
%\small{
\begin{tabular}{l|c|c|c}
\hline
Subset Size       & nGPU = 1 & nGPU=2 & nGPU=2 \\ 
 & LR = 1.0 & LR = 1.0 & LR = 2.0 \\
                    \hline \hline
                
0.1  & 11.26      & 13.99     & 11.32           \\
0.2 & 10.6        & 12.58    &  10.66      \\ 
0.3 & 10.4 & 11.58 & 10.46 \\\hline \hline     
\end{tabular}%}
\captionof{table}{\label{tab:ablation-3} Effect of Learning Rate on WER for \dsys{} on \textsc{test-clean} test set of Librispeech 100H.}
\end{table}


For the ASR task we recommend using at least 30\% of the dataset for training the model or using more warm-start epochs as described in Section~\ref{subsec:ablation}.
%\vspace{-.09cm}
In Table \ref{tab:wer_960}, we present comparison of the \dsys{} method with the baseline for the Librispeech 960H dataset on both the \textsc{test-clean} and \textsc{test-other} test sets. As shown in the Table, with just 30\% of the training data, \dsys{} is within 10\% of the relative test error (1\% of absolute error difference) when compared against training on the full data, thus yielding a speedup of 2.64. Similar results hold on the challenging \textsc{test-other} test set of the Librispeech which shows the better generalization of \dsys{} in comparison to the \random{} baseline. 

 \textbf{Results on Librispeech-noise}: We augment randomly selected signals from the dataset with noise across varying signal-to-noise ratios to mimic a more practical setting where subset selection algorithms need to address the noise while selecting useful subsets. We show the results on the Librispeech-noise 100H and 960H datasets for different subsets in Table \ref{tab:wer_noise}. \dsys{} consistently outperforms the \random{} baseline
 %\todo{We keep using "Random" very freely without necessarily qualiifying or reminding that is the Random-subset selection baseline
%Should we consider renaming "Random" consistently with "Random-subset"? Random-subset or something more appropriate}  
for different subsets with lower relative test error when compared against the full training and still yields significant speed up to reduce training time and maintain robustness.

\subsection{Ablation Study}
\label{subsec:ablation}

Next, we do an ablation study to understand the effect of learning rate on \dsys{} for Librispeech 100H dataset. Since, the goal of subset selection algorithms is to reduce the training data for training, the older recipes (especially learning rate) on full training data do not work  as-is for the \dsys{} because of the distributed nature of the training. 

In Table \ref{tab:ablation-3}, we show the effect of learning rate on multi-gpu training of the \dsys{} method. The recipe for single GPU borrowed as-is for the multi-gpu training setting, performed poorly because the number of gradient updates in the distributed setting halved. To overcome this barrier, we doubled the learning rate to take larger steps and reach convergence within the same number of epochs.



We perform some ablation studies to understand why subsets selected by \dsys{} tend to outperform a relatively simple \random{} baseline. We compute the following two metrics:

 \textbf{Overlap Index (OI)}: This is the fraction of common points selected in the last two subset selection rounds with the subset size. This metric computes the diversity of the points being selected by the methods in the subsequent subset selection rounds. 

 \textbf{Noise Overlap Index (NOI)}: This is the fraction of noise points selected by the subset selection methods divided by the total number of noisy points. Both the metrics are computed by averaging the index for all the runs with the same subset selection method.

% \begin{table}[h]
% \begin{tabular}{l|c|c}
%                     & Random Online & \multicolumn{1}{l}{\sys} \\ 
%                     \hline \hline
                
% Overlap Index       & 20.2\%       & 6.37\%                         \\
% Noise Overlap Index & 0.82\%        & 0.83\%               \\ \hline         
% \end{tabular}
% \caption{\label{tab:ablation-1} Overlap Indices for both the methods.}
% \vspace{-.65cm}
% \end{table}

 As shown in Table \ref{tab:ablation-1}, \dsys{} selects more diverse points across different subset selection rounds which explains the better generalization of the \textsc{test-other} test set. At the same time, both the methods select a similar amount of noisy points during the subset selection indicating that \dsys{} selects more diverse points from the non-noisy points.

 Finally, we study the effect of warm-start on the performance of the \dsys{} algorithm. Since it is an adaptive data selection algorithm, \dsys{}  needs a good starting point for computing reasonable estimates of the gradients for subset selection. Table \ref{tab:ablation-2} shows the effect of warm-start epoch ablation on the \textsc{test-clean} test set for Librispeech 960H. As we increase the warm start, the performance of the \dsys{} algorithm improves at the cost of  speed up. 

% \begin{table}[h]
% \begin{tabular}{c|c|c}
% Subset Size & WS = 2 epochs & WS= 3 epochs \\ \hline \hline
% 10\%        & 5.71                  & 5.3                   \\
% 20\%        & 5.01                  & 4.82                  \\
% 30\%        & 4.58                  & 4.54                 \\ \hline
% \end{tabular}
% \caption{\label{tab:ablation-2} Effect of warm start(WS) on WER for 960H}
% \vspace{-.65cm}
% \end{table}\noindent

\subsection{Comparing \dsys{} and \textsc{Grad-MatchPB}}

\begin{table*}[t]
    \centering
    \begin{tabular}{c| c| c| c| c| c} \hline 
     Subset-Size  & \random{} 	   & \largeSmall{} & \largeOnly & \textsc{Grad-MatchPB} & \dsys{}\\ \hline \hline
     
    0.1      & 16.64         & 17.98      &  17.27  & 16.14        & 16.23   \\
    0.2  & 16.43 & 17.23 &  16.35 & 15.89   & 16.03   \\
    0.3  & 16.28  & 16.35     &  16.22  & 15.79  & 15.95\\ \hline \hline
    \end{tabular}
    \caption{Comparison of WER obtained with  \random{}, \largeSmall{}, \largeOnly{},\textsc{Grad-MatchPB} and \dsys{} on TIMIT Phone recognition dataset.}
    \label{tab:pb_vs_pgm}
    
\end{table*}

Running \textsc{Grad-MatchPB} for Librispeech is prohibitively expensive since the amount of memory required to store all the gradients would exceed the memory size of available commercial GPUs as described in Section \ref{need}. To address this, we compare Phone Error (PER) on the TIMIT Phone recognition dataset \cite{garofolo1993timit} (containing 3680 utterances with 630 speakers) for all the methods. 
 
Table \ref{tab:pb_vs_pgm} shows WER obtained with \dsys{}, \textsc{Grad-MatchPB} \random{} and other subset selection baselines such as \largeSmall{}, \largeOnly{}. For \dsys{} we use data partitioning $D=2$. We see that the WER of \dsys{} is slightly higher than that of \textsc{Grad-MatchPB}, as the error term  that \dsys{} minimises is a upper bound of error term minimised by \textsc{Grad-MatchPB} as discussed in section \ref{conn_ew}. However, \dsys{}'s WER is very close to that of \textsc{Grad-MatchPB}, indicating that the partitioning doesn’t deteriorate the bounds while allowing to scale for larger datasets and utilize multiple GPUs which allows \dsys{} to enjoy better speedups over \textsc{Grad-MatchPB}.

\textbf{Statistical Significance: } WER reductions using \dsys{} compared to the \random{} baseline are statistically significant at $p < 0.001$ using a matched pairs test.\footnote{https://github.com/talhanai/wer-sigtest}



